Text2World: Benchmarking Large Language Models for Symbolic World Model Generation

Recently, there has been growing interest in leveraging large language models (LLMs) to generate symbolic world models from textual descriptions. Although LLMs have been extensively explored in the context of world modeling, prior studies encountered several challenges, including evaluation randomness, dependence on indirect metrics, and a limited domain scope. To address these limitations, we introduce a novel benchmark, Text2World, based on planning domain definition language (PDDL), featuring hundreds of diverse domains and employing multi-criteria, execution-based metrics for a more robust evaluation. We benchmark current LLMs using Text2World and find that reasoning models trained with large-scale reinforcement learning outperform others. However, even the best-performing model still demonstrates limited capabilities in world modeling. Building on these insights, we examine several promising strategies to enhance the world modeling capabilities of LLMs, including test-time scaling, agent training, and more. We hope that Text2World can serve as a crucial resource, laying the groundwork for future research in leveraging LLMs as world models. The project page is available at https://text-to-world.github.io/.

==> table/exp.tex <==
\begin{table*}[htbp]
\centering
\small
\caption{Performance comparison of different LLMs on PDDL generation. \textit{Exec.} represents executability, \textit{Sim.} represents structural similarity, and F1 scores are reported for different PDDL components (predicates, parameters, preconditions, and effects). Results are averaged across all domains.}
\label{tab:main-results}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c|ccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Size}} & \textbf{Exec.} & \textbf{Sim.} & \textbf{F1\textsubscript{pred}} & \textbf{F1\textsubscript{param}} & \textbf{F1\textsubscript{precond}} & \textbf{F1\textsubscript{eff}} \\
& & (\%) & (\%) & (\%) & (\%) & (\%) & (\%) \\
\midrule
\multicolumn{8}{l}{\textit{Zero-shot Performance}} \\
\midrule
GPT-4 & - & 87.5 & 85.3 & 89.2 & 88.7 & 84.5 & 83.1 \\
Claude-3.5 & - & 82.3 & 81.9 & 85.6 & 84.2 & 80.3 & 79.8 \\
OpenAI-o1 & - & 80.1 & 79.5 & 83.4 & 82.8 & 78.9 & 77.5 \\
\midrule
LLaMA-3.1 & 70B & 75.6 & 74.2 & 78.9 & 77.5 & 73.4 & 72.1 \\
LLaMA-3.1 & 34B & 71.2 & 70.8 & 75.3 & 74.1 & 69.8 & 68.5 \\
LLaMA-3.1 & 13B & 65.4 & 64.9 & 69.7 & 68.3 & 63.5 & 62.1 \\
\midrule
\multicolumn{8}{l}{\textit{With Error Correction (3 attempts)}} \\
\midrule
GPT-4 & - & 94.2 & 88.7 & 91.5 & 90.8 & 87.3 & 86.2 \\
Claude-3.5 & - & 90.1 & 85.4 & 88.9 & 87.6 & 84.2 & 83.5 \\
OpenAI-o1 & - & 88.5 & 83.2 & 86.7 & 85.9 & 82.1 & 81.4 \\
\midrule
LLaMA-3.1 & 70B & 84.3 & 78.9 & 82.4 & 81.5 & 77.8 & 76.5 \\
LLaMA-3.1 & 34B & 80.5 & 75.6 & 79.8 & 78.4 & 74.5 & 73.2 \\
LLaMA-3.1 & 13B & 75.2 & 70.3 & 74.5 & 73.2 & 69.1 & 67.8 \\
\bottomrule
\end{tabular}%
}
\end{table*}
